A Comprehensive Survey of Dynamic Graph Neural Networks: Models, Frameworks, Benchmarks, Experiments and Challenges

Dynamic Graph Neural Networks (GNNs) combine temporal information with GNNs to capture structural, temporal, and contextual relationships in dynamic graphs simultaneously, leading to enhanced performance in various applications. As the demand for dynamic GNNs continues to grow, numerous models and frameworks have emerged to cater to different application needs. There is a pressing need for a comprehensive survey that evaluates the performance, strengths, and limitations of various approaches in this domain. This paper aims to fill this gap by offering a thorough comparative analysis and experimental evaluation of dynamic GNNs. It covers 81 dynamic GNN models with a novel taxonomy, 12 dynamic GNN training frameworks, and commonly used benchmarks. We also conduct experimental results from testing representative nine dynamic GNN models and three frameworks on six standard graph datasets. Evaluation metrics focus on convergence accuracy, training efficiency, and GPU memory usage, enabling a thorough comparison of performance across various models and frameworks. From the analysis and evaluation results, we identify key challenges and offer principles for future research to enhance the design of models and frameworks in the dynamic GNNs field.

==> tex/application_domains.tex <==
% \documentclass[../main.tex]{subfiles}


% \begin{document}
% \label{Application}
% The dynamic graph representation learning algorithms mentioned above focus on specific domains or employ domain specific methods to solve dynamic graph problems. In section \ref{application_domains}, we will describe these algorithms combined with other fields.

% In addition, we will provide an overview of the application of dynamic graphs in different scenarios in Section \ref{diverse graphs}.

% \subsection{Application Domains}
% \label{application_domains}
% We divide these related algorithms into methods applied in the fields of transportation and recommendation systems, algorithms that use machine learning methods to complete dynamic graph tasks, and some other small parts that we will describe in the same section, as shown in Figure \ref{DGNN_domains}.

% \subsubsection{Transportation}
% Except GDCF\cite{GDCF} used for crowd flow prediction, STGNPP\cite{STGNPP} used for traffic congestion event prediction, the rest DGNN algorithm \cite{STGCN, T-GCN, MegaCRN, STWave} used for traffic prediction. STGCN\cite{STGCN} is the first application of pure convolution structure to extract spatio-temporal features from time series of graph structure in traffic research. T-GCN\cite{T-GCN} adopts GCN\cite{GCN} learning graph structure, and RNN learns time information from different graph snapshots, which can realize short-term prediction and long-term traffic tasks. GDCF provides a general and dynamic representation learning method for crowd flow modeling. STGNPP first uses the neural point process of a spatio-temporal map to predict traffic congestion events. MegaCRN\cite{MegaCRN} only depends on the observation data and is robust and adaptive to any traffic condition. STWave\cite{STWave} decouples complex traffic data into stable trend and fluctuation time and can capture the time variation and spatial correlation of two scales.

% \subsubsection{Recommendation Systems}
% The recommendation system is a very important part of social networks, and there have been many works designed for recommendation systems \cite{JODIE, HierTCN, DGCF, CDGP, TGRank, SUPA, DynShare, DGEL, DEGC}. JODIE\cite{JODIE} divides embedding into dynamic embedding and static embedding, learns time-varying and time-invariant features at the same time, and can model the future embedding trajectory of users/projects. HierTCN\cite{HierTCN} is a framework that can model large-scale data. The high-level model uses RNN to learn long-term interest, and the low-level model uses TCN\cite{TCN} to predict the next interaction using long-term interest and short-term interaction. DGCF\cite{DGCF} can effectively model the dynamic relationship between users and projects, and can simultaneously capture the collaborative and sequential relationship between projects and users. CDGP\cite{CDGP} is a learning method based on a community dynamic graph for popularity prediction. It designs a community detection module to capture the evolving community structure. TGRank\cite{TGRank} enhances the expression ability in link prediction and can calculate listwise losses in link prediction of large candidate sets. SUPA\cite{SUPA} can link neighborhood interference, which is a way to expand to large dynamic graphs. DynShare\cite{DynShare} has improved Jodie's time projection module to sense the time interval. DGEL\cite{DGEL} designs a three process, which can comprehensively update the dynamic embedding of nodes with rich graph information.DEGC\cite{DEGC} models temporal user preferences as user embedded initialization to help learn user preferences for emerging data.

% \subsubsection{Machine Learning Methods}
% Some work uses machine learning methods or ideas to help implement dynamic graph algorithms. \cite{SGNN-GR,DEGC,PI-GNN} adopt the idea of continuous learning. SGNN-GR\cite{SGNN-GR} uses GAN\cite{GAN} to generate false historical sample data, which can avoid catastrophic forgetting without saving additional data. DEGC\cite{DEGC} is a continual graph learning method based on model isolation\cite{modelIsolation1,modelIsolation2}. PI-GNN\cite{PI-GNN} learns new patterns by isolating stable parameters\cite{parameter} and expanding parameters to reduce catastrophic forgetting. WinGNN\cite{WinGNN} uses a meta-learning strategy to model the adjacent and continuous snapshots in the sliding window and can learn the information of different time scales. DREAM\cite{DREAM} designed an adaptive reinforcement learning framework to predict missing elements by learning adaptive rewards at the semantic and temporal rule levels.

% \subsubsection{Others}
% \cite{Netwalk, AER-AD, LRGCN} is a method used for anomaly detection. Netwalk\cite{Netwalk} can detect anomalous vertices and edges that may evolve in the network by dynamically inserting or deleting them. AER-AD\cite{AER-AD} can perform anomaly detection in dynamic bipartite graphs in an inductive environment. LRGCN\cite{LRGCN} is used for path fault prediction and a self-attention path embedding module is designed for it. \cite{APAN, RT-GCN} are DGNN algorithms in the financial field. APAN\cite{APAN} adopts asynchronous processing methods, which can detect financial fraud on time. RT-GCN\cite{RT-GCN} is used for ranking-based stock prediction tasks, which models the relationship and time characteristics between each stock as a relationship time graph to explore the relationships between different stocks. TEDIC\cite{TEDIC} is used in social interaction networks to extract patterns from dynamic social interactions. TFE-GNN\cite{TFE-GNN} provides support from different perspectives for encrypted traffic classification.

% \begin{figure*}
% 	\centering 
% 	\includegraphics[width=0.8\textwidth, angle=0]{fig/domains.pdf}	
%     \vspace{-10pt}
% 	\caption{The summary of the different application domains of DGNN in our survey} 
% 	\label{DGNN_domains}%
% \end{figure*}

% \subsection{Graphs in Different Scenarios}
% \label{diverse graphs}
% In this section, we have summarized the DGNN algorithms used for different types of graphs. The overview of the entire classification is shown in Figure \ref{DGNN_scenairos}.

% \textbf{Temporal Knowledge graph.} \cite{Know-E, RE-Net, GHN, TeMP, DREAM, RPC, RETIA} are all algorithms designed for temporal knowledge graphs. These algorithms are essentially no different from those used for ordinary dynamic graphs, except that they may have been specially processed due to the characteristics of knowledge graphs.

% \textbf{Temporal heterogeneous graph.}\cite{HDGNN, DyHATR, RISD, SUPA, RETIA, LRGCN, TeMP, OTGNet} are algorithms used for heterogeneous graphs. For graphs with heterogeneous edges, an intuitive approach is to use R-GCN to directly process the graph structure. However, there are also algorithms specifically designed for heterogeneous graphs. This algorithm usually takes more time, but it also has better performance.

% \textbf{Spatio-Temporal graph.}The algorithms used for spatio-temporal graphs include \cite{SSGNN, STGNPP, STGNP, MegaCRN, STWave, STGCN}. Most spatio-temporal maps are often related to the field of transportation and are commonly used for predicting traffic neighborhoods.

% \textbf{Directed acyclic graph(DAG).}\cite{GraphNOTEARS} is an algorithm used for DAG representation learning problems, and there have been few previous works that have linked this aspect to DGNN algorithms.

% \begin{figure}
% 	\centering 
% 	\includegraphics[width=0.5\textwidth, angle=0]{fig/diverse_type.pdf}	
% 	\caption{DGNN in different scenairos} 
% 	\label{DGNN_scenairos}%
% \end{figure}

% \end{document}

